Transverse Resummation for Direct Photon Production

Quantum Chromodynamics predicts radiative terms which, at low transverse momentum of an observed multi-particle system, can be large enough to threaten the legitimacy of a fixed-order perturbative treatment. We present a subtraction-style calculation which sums these terms to all orders for a direct photon plus jet final state, and show that the kinematic effect of such a resummation is significant even after integration over the jet. An improved matching algorithm is prescribed for the transition to the perturbative regime, and re-examination of the nonperturbative regime indicates that simple Gaussian parametrizations are to be favored, with coefficients that depend not on the photon-jet mass, but on the color structure of the initiated subprocess. Agreement with data is significantly improved, and the method is expected to have applicability in general for processes with steeply-falling spectra.

==> finkdefs.tex <==
\makeatletter
\def\pmb#1{\leavevmode\setbox0=\hbox{#1}%
\kern-.02em\copy0\kern-\wd0
\kern.04em\copy0\kern-\wd0
\kern-.02em\raise.04em\box0 }

\usepackage{feynmf}  %Formerly rem'd out in original.
\unitlength=1mm
%\usepackage[dvips]{graphics}
%\usepackage{rotating}
\definecolor{green4}{rgb}{0,.54,0}
\definecolor{orangered}{rgb}{1,.27,0}


\def\notA{{\hbox{$A$}\kern-5.87pt{/}\ }}
\def\notD{{\hbox{$D$}\kern-7.37pt{/}\ }}
\def\notcalD{{\hbox{${\cal D}$}\kern-6.87pt{/}\ }}
\def\notcalA{{\hbox{${\cal A}$}\kern-6.87pt{/}\ }}
\def\notp{{\hbox{$p$}\kern-5.87pt{/}\ }}
\def\notpartial{{\hbox{$\partial$}\kern-5.87pt{/}\ }}
\def\notDO{{\hbox{O}\kern-7.37pt{/}\ }}

%%% New commands by Chris Fink:
\newcommand{\figboxf}[2]{\begin{figure}[h]\centering \begin{minipage}{\linewidth}
\centering \epsfxsize = \linewidth \leavevmode\epsffile{#1.eps}
\end{minipage} \caption[#2]{#2} \label{fig:#1} \end{figure} }

\newcommand{\figboxh}[2]{\begin{figure}[h]\centering \begin{minipage}{\linewidth}
\centering \epsfxsize = 0.5\linewidth \leavevmode\epsffile{#1.eps}
\end{minipage} \caption[#2]{#2} \label{fig:#1} \end{figure} }

\newcommand{\figboxa}[2]{\begin{figure}[h]\centering \begin{minipage}{\linewidth}
\centering \epsfxsize = 0.75\linewidth
\leavevmode\epsffile{#1.eps}
\end{minipage} \caption[#2]{#2} \label{fig:#1} \end{figure} }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\entrylabel}[1]{\mbox{\textsf{#1:}}\hfil}
\newenvironment{entry}%
 {\begin{list}{}%
   {\renewcommand{\makelabel}{\entrylabel}%
    \setlength{\labelwidth}{3cm}%
    \setlength{\leftmargin}{1.25in}
%    \setlength{\rightmargin}{1in}
   }%
 }%
{\end{list}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% begin new commands from Joergen Beck Hanson
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\BQA}     {\begin{eqnarray}}
\newcommand{\EQA}     {\end{eqnarray} \noindent}
\newcommand{\BQN}     {\begin{equation}}
\newcommand{\EQN}     {\end{equation} \noindent}
\newcommand{\BFIG}     {\begin{figure}[h]\centering}
\newcommand{\EFIG}     {\end{figure}}
\newcommand{\BEQNA}    {\renewcommand{\arraystretch}{1.75}\begin{equation}\begin{array}{rcl}}
\newcommand{\EEQNA}    {\end{array}\end{equation}\renewcommand{\arraystretch}{1}}
\newcommand{\refmat}[1]   {equation~\ref{#1}}
\newcommand{\reffig}[1]   {figure~\ref{#1}}
\newcommand{\reftab}[1]   {table~\ref{#1}}
\newcommand{\mw}       {\mbox{$ {\mathrm M}_{\mathrm W}$}}
\newcommand{\gw}       {\mbox{$ \Gamma_{\mathrm W}$}}
\newcommand{\mz}       {\mbox{$ {\mathrm M}_{\mathrm Z}$}}
\newcommand{\mws}       {\mbox{$ {\mathrm M}_{\mathrm W}^2$}}
\newcommand{\mzs}       {\mbox{$ {\mathrm M}_{\mathrm Z}^2$}}
\newcommand{\mh}       {\mbox{$ {\mathrm M}_{\mathrm H}$}}
\newcommand{\mt}       {\mbox{$ {\mathrm M}_{\mathrm t}$}}
\newcommand{\w}        {\mbox{$ {\mathrm W}$}}
\newcommand{\Wp}       {\mbox{$ {\mathrm W}^+ $}}
\newcommand{\Wm}       {\mbox{$ {\mathrm W}^- $}}
\newcommand{\wpm}      {\mbox{$ {\mathrm W}^{\pm} $}}
\newcommand{\photon}   {\mbox{$ \gamma$}}
\newcommand{\A}        {\mbox{$ {\mathrm A}$}}
\newcommand{\z}        {\mbox{$ {\mathrm Z}^0$}}
\newcommand{\ee}       {\mbox{$ {\mathrm e}^+ {\mathrm e}^-$}}
\newcommand{\ww}       {\mbox{$ {\mathrm W}^+ {\mathrm W}^-$}}
\newcommand{\zz}       {\mbox{$ {\mathrm Z}^0 {\mathrm Z}^0$}}
\newcommand{\wz}       {\mbox{$ \z \w$}}
\newcommand{\wwz}      {\mbox{$ \z \ww$}}
\newcommand{\wwgamma}  {\mbox{$ \gamma \ww$}}
\newcommand{\eeff}     {\mbox{$ \ee \rightarrow {\mathrm f} \bar{{\mathrm f}}$}}
\newcommand{\eezgammaff}     {\mbox{$ \ee \rightarrow \z /\photon \rightarrow
    {\mathrm f} \bar{{\mathrm f}}$}}
\newcommand{\eeffff}   {\mbox{$ \ee \rightarrow {\mathrm f}_1 \bar{{\mathrm
        f}_2} {\mathrm f}_3 \bar{{\mathrm f}_4} $}}
\newcommand{\eewwffff} {\mbox{$ \ee \rightarrow \ww \rightarrow {\mathrm f}_1
    \bar{{\mathrm f}_2} {\mathrm f}_3 \bar{{\mathrm f}_4} $}}
\newcommand{\eeww}     {\mbox{$ \ee \rightarrow \ww$}}
\newcommand{\wwqqlv}   {\mbox{$ \ww \rightarrow qq \ell \nu $}}
\newcommand{\wwjjlv}   {\mbox{$ \ww \rightarrow jj \ell \nu $}}
\newcommand{\wwjjev}   {\mbox{$ \ww \rightarrow jj e \nu $}}
\newcommand{\wwjjmv}   {\mbox{$ \ww \rightarrow jj \mu \nu $}}
\newcommand{\wwjjjj}   {\mbox{$ \ww \rightarrow jjjj$}}
\newcommand{\lvlv}     {\mbox{$ \ell \nu \ell \nu$}}
\newcommand{\lvqq}     {\mbox{$ \ell \nu q \bar{q}$}}
\newcommand{\evqq}     {\mbox{$ e \nu q \bar{q}$}}
\newcommand{\muvqq}     {\mbox{$ \mu \nu q \bar{q}$}}
\newcommand{\lvjj}     {\mbox{$ \ell \nu j j$}}
\newcommand{\evjj}     {\mbox{$ e\nu jj$}}
\newcommand{\muvjj}     {\mbox{$ \mu\nu jj$}}
\newcommand{\jjev}     {\mbox{$jj e\nu$}}
\newcommand{\jjmv}     {\mbox{$jj\mu\nu$}}
\newcommand{\tauvjj}     {\mbox{$ \tau\nu jj$}}
\newcommand{\evev}     {\mbox{$ e\nu e\nu $}}
\newcommand{\evmuv}     {\mbox{$ e\nu \mu\nu $}}
\newcommand{\evtauv}     {\mbox{$ e\nu \tau\nu $}}
\newcommand{\muvmuv}     {\mbox{$ \mu\nu \mu\nu $}}
\newcommand{\muvtauv}     {\mbox{$ \mu\nu \tau\nu $}}
\newcommand{\tauvtauv}     {\mbox{$ \tau\nu \tau\nu $}}
\newcommand{\eeee}     {\mbox{$ \ee\ee$}}
\newcommand{\evud}     {\mbox{$ {\mathrm e}^- \bar{\nu}_e {\mathrm u}
    \bar{{\mathrm d}}$}}
\newcommand{\qqqq}     {\mbox{$ q q q q$}}
\newcommand{\jjjj}     {\mbox{$ j j j j$}}
\newcommand{\ppbar}    {\mbox{$ {\mathrm p} \bar{{\mathrm p}} $}}
\newcommand{\pantip}   {\mbox{$ {\mathrm p} \bar{{\mathrm p}} $}}
\newcommand{\gev}      {\mbox{GeV}}
\newcommand{\mev}      {\mbox{MeV}}
\newcommand{\tev}      {\mbox{TeV}}
\newcommand{\nb}       {\mbox{nb}}
\newcommand{\nbinv}    {\mbox{nb$^{-1}$}}
\newcommand{\pb}       {\mbox{pb}}
\newcommand{\pbinv}    {\mbox{pb$^{-1}$}}
\newcommand{\pantiptowgamma}      {\mbox{$ \pantip\rightarrow\w\gamma $}}
\newcommand{\lv}       {\mbox{$ \ell \nu$}}
\newcommand{\qqbar}    {\mbox{$ q \bar{q}$}}
\newcommand{\vt}       {\vartheta}
\newcommand{\kg}{\kappa_\gamma}
\newcommand{\kZ}{\kappa_Z}
\newcommand{\lmg}{\lambda_\gamma}
\newcommand{\lZ}{\lambda_Z}
\newcommand{\dZ}{\delta_Z}
\newcommand{\xg}{x_\gamma}
\newcommand{\xZ}{x_Z}
\newcommand{\yg}{y_\gamma}
\newcommand{\yZ}{y_Z}
\newcommand{\pvl}{{\vec p}_l}
\newcommand{\pvlb}{{\vec p}_{\bar{l}}}
\newcommand{\pvn}{{\vec p}_{\nu}}
\newcommand{\pvnb}{{\vec p}_{\bar{\nu}}}



%Standard journal references
\def\ap#1#2#3   {{\em Ann. Phys. (NY)} {\bf#1} (#2) #3.}
\def\apj#1#2#3  {{\em Astrophys. J.} {\bf#1} (#2) #3.}
\def\apjl#1#2#3 {{\em Astrophys. J. Lett.} {\bf#1} (#2) #3.}
\def\app#1#2#3  {{\em Acta. Phys. Pol.} {\bf#1} (#2) #3.}
\def\ar#1#2#3   {{\em Ann. Rev. Nucl. Part. Sci.} {\bf#1} (#2) #3.}
\def\cpc#1#2#3  {{\em Computer Phys. Comm.} {\bf#1} (#2) #3.}
\def\err#1#2#3  {{\it Erratum} {\bf#1} (#2) #3.}
\def\ib#1#2#3   {{\it ibid.} {\bf#1} (#2) #3.}
\def\jmp#1#2#3  {{\em J. Math. Phys.} {\bf#1} (#2) #3.}
\def\ijmp#1#2#3 {{\em Int. J. Mod. Phys.} {\bf#1} (#2) #3.}
\def\jetp#1#2#3 {{\em JETP Lett.} {\bf#1} (#2) #3.}
\def\jpg#1#2#3  {{\em J. Phys. G.} {\bf#1} (#2) #3.}
\def\mpl#1#2#3  {{\em Mod. Phys. Lett.} {\bf#1} (#2) #3.}
\def\nat#1#2#3  {{\em Nature (London)} {\bf#1} (#2) #3.}
\def\nc#1#2#3   {{\em Nuovo Cim.} {\bf#1} (#2) #3.}
\def\nim#1#2#3  {{\em Nucl. Instr. Meth.} {\bf#1} (#2) #3.}
\def\np#1#2#3   {{\em Nucl. Phys.} {\bf#1} (#2) #3.}
\def\pcps#1#2#3 {{\em Proc. Cam. Phil. Soc.} {\bf#1} (#2) #3.}
\def\pl#1#2#3   {{\em Phys. Lett.} {\bf#1} (#2) #3.}
\def\prep#1#2#3 {{\em Phys. Rep.} {\bf#1} (#2) #3.}
\def\prev#1#2#3 {{\em Phys. Rev.} {\bf#1} (#2) #3.}
\def\prl#1#2#3  {{\em Phys. Rev. Lett.} {\bf#1} (#2) #3.}
\def\prs#1#2#3  {{\em Proc. Roy. Soc.} {\bf#1} (#2) #3.}
\def\ptp#1#2#3  {{\em Prog. Th. Phys.} {\bf#1} (#2) #3.}
\def\ps#1#2#3   {{\em Physica Scripta} {\bf#1} (#2) #3.}
\def\rmp#1#2#3  {{\em Rev. Mod. Phys.} {\bf#1} (#2) #3.}
\def\rpp#1#2#3  {{\em Rep. Prog. Phys.} {\bf#1} (#2) #3.}
\def\sjnp#1#2#3 {{\em Sov. J. Nucl. Phys.} {\bf#1} (#2) #3.}
\def\spj#1#2#3  {{\em Sov. Phys. JEPT} {\bf#1} (#2) #3.}
\def\spu#1#2#3  {{\em Sov. Phys.-Usp.} {\bf#1} (#2) #3.}
\def\zp#1#2#3   {{\em Zeit. Phys.} {\bf#1} (#2) #3.}

\newcommand{\putpicture}[3]{%
\IfFileExists{#3}{\resizebox{#1}{#2}{\includegraphics{#3}}}
 {\resizebox{#1}{#2}{File
   #3 \\ is missing}}
}
\newcommand{\putpic}[1]{
  \IfFileExists{#1}{\includegraphics{#1}}
 {\resizebox{5cm}{5cm}{File
   #1 \\ is missing}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% end from Joergen Beck Hanson
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\makeatother

\widowpenalty=10000
\clubpenalty=10000
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.5}
\renewcommand{\floatpagefraction}{0.8}
\renewcommand{\textfraction}{0.1}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}
\pretolerance=500
\tolerance=1000
\hbadness=3000
\vbadness=3000
\hyphenpenalty=400

%%%  some struts for tables  (mimi)
\newcommand{\strutrule}{\vrule height16pt width0pt depth9pt}
\newcommand{\ruleup}{\vrule height16pt width0pt depth0pt}
\newcommand{\bigruleup}{\vrule height20pt width0pt depth0pt}
\newcommand{\ruledown}{\vrule height0pt width0pt depth10pt}
\newcommand{\bigruledown}{\vrule height0pt width0pt depth20pt}


\endinput

